CM-GAN: Image Inpainting with Cascaded Modulation GAN and Object-Aware Training

Recent image inpainting methods have made great progress but often struggle to generate plausible image structures when dealing with large holes in complex images. This is partially due to the lack of effective network structures that can capture both the long-range dependency and high-level semantics of an image. We propose cascaded modulation GAN (CM-GAN), a new network design consisting of an encoder with Fourier convolution blocks that extract multi-scale feature representations from the input image with holes and a dual-stream decoder with a novel cascaded global-spatial modulation block at each scale level. In each decoder block, global modulation is first applied to perform coarse and semantic-aware structure synthesis, followed by spatial modulation to further adjust the feature map in a spatially adaptive fashion. In addition, we design an object-aware training scheme to prevent the network from hallucinating new objects inside holes, fulfilling the needs of object removal tasks in real-world scenarios. Extensive experiments are conducted to show that our method significantly outperforms existing methods in both quantitative and qualitative evaluation. Please refer to the project page: \url{https://github.com/htzheng/CM-GAN-Inpainting}.

==> sections/intro_old.tex <==
% stylegan 对不align的结果不好,因为不align,缺少spatial信息,基于这个motivation,为了更好利用structural information, (stlyegan global modulation + skip connection; comodgan没法利用洞里面的spatial信息,sturcure不对),我们用前一个layer的的sturcutal信息,利用spatial modulation,提供更好的结果信息.用了不光是global 信息,也用了local信息,保证structural更对. (skip connection提供structure信息)

% 跟stylemapgan的区别
% cascade modulation 的作用,更好的refine structure,再用global information,交替性的update洞里的信息,用global code check对不对
% global modulation结果作为latern style code

\section{Introduction}
Image inpainting refers to the task of completing missing regions of an image. As an important computer vision problem, it has many practical applications, such as removing distracting objects from of an image, image re-targeting, image composition and many others.

Early works on image inpainting rely on patch-based copy-pasting strategies~\cite{patchmatch,kwatra2005texture,cho2008patch} to borrow patches from known regions or solving partial differential equations~\cite{ballester2001filling,chan2001nontexture,shen2002mathematical,criminisi2004region} to propagate pixel values to the missing region. Those methods are quite effective for generating stationary textures or completing simple shapes, but they cannot hallucinate new textures or image structures. 

With the advancement of deep learning and generative models, research efforts have largely shifted to solving inpainting as an end-to-end learning task where feed-forward generative models are trained to predict the completed image from an input image with masked area. 
% Compared to the traditional methods,
By training deep generative networks with adversarial losses~\cite{gan}, the learning-based approaches can leverage semantic information learned from large image sets to hallucinate better semantic structures, thus producing more appealing results.
% With the development of deep learning, inpainting has shifted to data-driven paradigm~\cite{} where neural networks are learned to directly predict inpainting results from the masked images. Trained with adversarial loss~\cite{gan} on large , those methods can produce more plausible outputs and significantly improve the image inpainting quality. Those methods often produce visual artifacts, especially when the hole is large.

% Despite the past progress on the subject, how to fill in the missing region with sensible and coherent content remains a huge challenge, due to insufficent . To model the long range dependency,

However, designing an inpainting network that produces both \emph{coherent} and \emph{plausible} contents is challenging.
Essentially, a generator needs to model the long range dependency of an image such that the generated content is consistent to the contextual clues outside the holes.\zl{we may need other recent references too, e.g. DeepFill-v2, ProFill} \hz{revised} Existing works rely on two-stage networks~\cite{deepfill,MEDFE,deepfillv2}, attention, Fourier convolution~\cite{lama} or iterative hole filling~\cite{profill} to propagate contextual features for generating coherent output. However, those methods are limited at reconstructing high-level structures, since their bottleneck layers are not designed to capture global semantics. To improve the generation capacity of a model, a recent work~\cite{comodgan} leverages global code to modulate StyleGAN2~\cite{stylegan2} blocks for inpainting and achieves impressive results. However, the model tends to generate incoherent outputs, such as distorted textures, color blobs, fake objects due to lack of mechanisms to correct incoherent features inside the hole.

\hz{revised} Another key component to inpainting is a properly designed training objective. While the adversarial training loss~\cite{gan} can improve the realism of inpainting, existing works~\cite{deepfill,deepfillv2,lama,profill,edgeconnect} rely on reconstruction loss such as l1 loss and perceptual loss and contextual loss to suppress artifacts. However, those methods are prone to produce overly smooth results and the reconstruction loss need to be carefully tuned.
Based on a strong discriminator, a recent work~\cite{comodgan} propose to use only the adversarial loss to encourage the diversity and realism of the output. However, as their randomly sampled mask often covers objects, the trained model often produce fake objects and color blobs inside the hole.

In this paper, we aims to improve both the network design and the training scheme for building image inpainting models tailored for real-world applications, such as object removal.
On the architecture side, we leverage global code modulation~\cite{stylegan2,comodgan} to model the global-range structure of an image. However, unlike~\cite{comodgan},  we propose a cascaded modulation design that serves to refine the internal feature maps in a coarse-to-fine manner. To improve the consistency of intermediate feature maps inside the hole, we further propose spatially adaptive demodulation to spatially modulate the fine stage features. Finally, we leverage fast Fourier convolutions to expand the receptive field of network at early stages, making the network better at modeling the global structure of an image.

On the loss side, we design an object-aware mask generation scheme. By avoiding cases where the full or majority of an object are covered by the mask, the trained model is less prone to generating fake new objects \jz{object blobs?}, allowing the model to be more suitable for training with only GAN losses for realistic image generation. Furthermore, we proposed a masked $R_1$ regularization that is specifically design to stabilize the training of inpainting network.

Our main key contribution are four-fold:
\begin{itemize}[noitemsep]
    \item We propose a new network design the cascades global code modulation with spatial modulation for robust image inpainting.
    
    \item We propose an object-aware scheme to synthesize training data for real object removal and partial object completion.
    
    \item We propose a masked $R_1$ loss to stabilize the adversarial training of image inpainting task.
    
    \item We achieves the state-of-the-art performance on the Places2 dataset under various setting.
\end{itemize}

==> sections/method_old.tex <==
% \section{Notation for Figure}
% \begin{align*}
% \large
% \vz \sim \mathcal{N}(0,\,\vI)\,\\
% \vz \in \sZ\\
% \vw \in \sW \\
% \vg \\
% \ve \\
% \vs \\
% (\vx, \vx \odot \vm) \\
% [\vx; \vx \odot \vm] \\
% [\vx \odot (1-\vm);\vm] \\
% \sR^{C\times H\times W}\\
% \sR^{C\times H\times W}\\
% [\vw;\vg] \in \sR^{N_w+N_g}\\
% \tF_e^{\text{in}}\\
% \tF_g^{\text{in}}\\
% \tF_g^{\text{out}}\\
% \tF_{gl}^{\text{in}}\\
% \tF_{gl}^{\text{out}}\\
% \vx^{(t)}\\
% \vx^{(t+1)}\\
% \vy\\
% \end{align*}

\section{Method}\label{sec:methodology}
Image inpainting aims to complete the missing region of an image $x$ annotated by a binary mask $m$.
While existing works have shown promising results~\cite{deepfill,deepfillv2,profill,comodgan} on hallucinating local textures and simple structures, generating plausible holistic structures while maintaining high-fidelity local details for complex scene remains a fundamental challenge.
Moreover, the possible suspicious artifact, i.e. distorted objects or color blobs would easily exacerbate visual quality under real use case.
We discover that a new mechanism named \emph{global-local cascaded modulation} and the consequent Cascaded Modulation GAN (CM-GAN) (\cref{sec:cmgan})
% a new way to perform feature modulation~\cite{spade,stylegan,stylegan2,stylemapgan},
% to introduce global-local interaction
has a profound effect on how the global context interact and propagated to local details and it leads to significantly better holistic structure and local details.
We also found that the tendency to generate suspicious objects and blobs can be further addressed by a proper and more generalizable object-aware training scheme (\cref{sec:mask_scheme}).
Finally, we propose the training objective stabilized by a masked $R_1$ regularization (\cref{sec:masked_r1}).
% Consequently, we propose: i) a new inpainting network named Cascaded Modulation GAN (CM-GAN) (\cref{sec:cmgan}), ii) an object-ware training scheme (\cref{sec:mask_scheme}), and iii) the training objective stabilized by a masked $R_1$ regularization (\cref{sec:masked_r1}).


\subsection{The Cascaded Modulation GAN}\label{sec:cmgan}
The Cascaded Modulation GAN (CM-GAN) is based on the principle of \emph{global-local cascaded modulation} and to introduce enhanced global-local interaction and Fast Fourier convolution~\cite{chi2020fast} to expand the recept field.
With such a design, the CM-GAN is a simple

CM-GAN is simple yet strong model based on the encoder-decoder structure, which is vastly different from  
Different from the existing mechanisms based two-stage network~\cite{}, dilated convolution or attention, we starts from 

single-pass modulation[56], multi-stage image-refinement [33,47,52] or feature propagation via dilated-conv [52] / attention [50]

For the task, GANs~\cite{gan} leverage a generator $\mathcal{G}$ that predicts the final outcome $\hat{x}$ from the incomplete image $x\odot m$, the mask $m$ as well as a Gaussian noise vector $\vz \sim \mathcal{N}(\mathbf{0},\mI)$
\begin{align}
\label{eq:G}
\begin{aligned}
    \hat{x} = \mathcal{G}(x\odot m,\,m,\,\vz),
\end{aligned}
\end{align}
a discriminator $\mathcal{D}$ that predicts how likely outcome $\hat{x}$ is the ground truth.



\noindent \textbf{Network Overview.} \quad 
As shown in \cref{fig:network} (left), the Cascased Modulation GAN (CM-GAN) is

based on the cascaded modulation (CM) design that progressively upsample the encoded features for image inpainting. 
The CM leverage a sequence of paralleled global blocks and global-local blocks to predict global structure while enhance local details. By bridging global context with style code-based global modulation~\cite{stylegan} and introducing the global-local interaction with 

To facilitate visual quality of holistic and local details


a sequence of paralleled global blocks and global-local blocks to progressively upsample features. Both global and global-local blocks leverage a global code for 

More specifically, CM-GAN starts with an encoder $E$ that takes the partial image and the mask as inputs to produce multi-scale feature maps:
\begin{align}
\label{eq:encoder}
\begin{aligned}
    \tF_e^{(1)},\cdots,\tF_e^{(L)} = E(x \odot (1-m), m),
\end{aligned}
\end{align}
where $\tF_e^{(i)}$ are the generated feature at scale $1 \le i \le L$ ($L$ is the highest scale). The encoder is implemented by strided convolutions with residual connection.

\begin{figure}[t]
	\centering
% 	\includegraphics[width=0.5\linewidth]{figures/pipeline_v3.pdf}
	\includegraphics[width=1.0\linewidth]{figures/block_v5_eccv.pdf}
	\caption{
% 	The encoder-decoder network for inpainting.
    \textbf{Left}: CM-GAN consists of paralleled \textbf{\textcolor{cyan}{global blocks}} and \textbf{\textcolor{blue}{global-local blocks}} that progressive upsample features by modulating from a global code $\vg$.
    We propose \emph{cascaded modulation} that connects the two blocks with the introduced globally-aware and spatially-adaptive modulation, which brings high-order and global-local interaction for better inpainting. \textbf{Right}: Cascaded modulation at each scale.
    Its global and global-local blocks takes $\tF_g^{\text{in}}$ and $\tF_g^{\text{in}}$, respectively, as inputs and produce the upsampled versions $\tF_g^{\text{out}}$ and $\tF_g^{\text{out}}$.
    We propose global-spatial fusion, spatial modulation and normalization (\textbf{sMod std} and \textbf{sNorm std}) to enable the StyleGAN2-compatible cascaded modulation.
	}
	\label{fig:network}
	\vspace*{-.15in}
\end{figure}

% In fact, most prior works on inpainting are based on encoder-decoder architecture, such as CoModGAN(ICLR'21), LaMa(WACV'21), ProFill(ECCV'20), HiFIll(CVPR'20), DeepFillv2(ICCV'19).

To better inject global information while facilitating image synthesis, we computes a global code for feature modulation~\cite{stylegan,stylegan2}. we computes a global style code from highest scale feature $\mF_e^{(L)}$, a fully connected layer followed by a $\ell_2$ normalization produces a global style code $\vs = \fc(\mF_e^{(L)}) / \norm{\fc(\mF_e^{(L)})}_2$ to represent the input globally.
% , specifically,
% \begin{align}
% \label{eq:fc}
% \begin{aligned}
%     \vs = \fc(\mF_e^{(L)}) / (\norm{\fc(\mF_e^{(L)})}^2+\epsilon),
% \end{aligned}
% \end{align}
% where $\epsilon=10^{-5}$ is a small number to avoid dividing by zero.
In parallel to the encoder, a MLP-based mapping network~\cite{stylegan2} produces a random style code $\vw$ from a normalized random Gaussian noise $\rz$, simulating the stochasticity of the generation process. 
As suggested by~\cite{comodgan}, $\vw$ is joined with $\vs$ to produce the final global code $\vg=[\vs;\,\vw]$ for decoding. 
% \jz{Shall we add $s$ to Fig.~\ref{fig:network}?}

% , resulting a global code $\vg$ that represents both the global information and random variation of the output image, specifically:
% \begin{align}
% \label{eq:global_code}
% \begin{aligned}
%     \vg=[\vs;\,\vw].
% \end{aligned}
% \end{align}


% \iffalse
Next, as illustrated in \cref{fig:network} (right), the decoder is based on stacks a sequence of cascaded modulation blocks to upsample the input feature map $\mF_e^{(L)}$.
Motivated by feature modulation~\cite{stylegan,stylegan2}, each cascaded modulation block takes the global code $\vg$ as input to modulate the feature according to the global representation of the partial image.
However, our approach differs from the existing methods as the cascaded modulation block provides mechanisms to correct local error after predicting the global structure.
% \fi

\noindent \textbf{Cascaded Modulation Block.} \quad 
we propose a \emph{cascaded modulation} block (\cref{fig:network} (right)) to address the challenge of generating coherent features both globally and locally.
% in comparison to the StyleGAN2-based global code modulation (right)
At a high level, it follows the principles of: i) a decomposition of global and local features to separate local details from global structure, ii) a cascade of global and spatial modulation that predicts local details from global structures. Unlike existing spatial modulation approaches~\cite{stylemapgan,spade}, our proposed spatial modulation utilizes the global code for better prediction and discards the instance normalization to make the design compatible with StyleGAN2~\cite{stylegan2}.

More specifically, the cascaded modulation takes the global and local feature $\tF_g^{(i)}$ and $\tF_l^{(i)}$ from previous scale and the global code $\vg$ as input and produces the new global and local features $\tF_g^{(i+1)}$ and $\tF_g^{(i+1)}$ at next scale.
To produce the new global code $\tF_g^{(i+1)}$ from $\tF_g^{(i+1)}$, a global code modulation stage is proposed that repeats the ``modulation-convolution-demodulation'' procedure of StyleGAN2~\cite{stylegan2} (illustrated in global block of \cref{fig:network}) to generate a upsampled feature $\tX$ and the a global code. However, we remove all the broadcast noise from the global modulation block and leave it to the spatial modulation stage.

% \begin{figure}[t]
% 	\centering
% 	\includegraphics[width=0.5\linewidth]{figures/block_v4.pdf}
% 	\caption{The cascaded modulation applies \emph{global modulation} first on the global feature map $\tF_g$ (left) and then apply \emph{spatial modulation} on the local feature map $\tF_l$ (right) and the output is passed down to their corresponding next level blocks, respectively. We propose spatial modulation (\textbf{sMod std}) and normalization (\textbf{sNorm std}) to enable the StyleGAN2-compatible spatial modulation.
% % 	\todo{$tA_0$ is not reflected in Fig}
% % 	\todo{add input output illstration, input Fg, Fl, Fe, output Fg, Fl}
% % 	\todo{F_in and F_out}
% % The spatial modulation takes both spatial feature $\tX$ and global code $\vg$ as inputs and applies spatial feature modulation (\textbf{sMod std}) and normalization respectively) to generate the modulated output.
% % Left: StyleGAN2-based modulation~\cite{stylegan2} takes a global code as input to modulate features. Right: cascaded modulation which applies global modulation first on the input feature map and then apply spatial modulation on top, and both globally modulated feature maps ($out\_{global} X$) and spatially modulated feature maps ($out\_{local} Y$) are passed down to their corresponding next level blocks, respectively. 
% 	}
% 	\label{fig:modulation}
% 	\vspace*{-.15in}
% \end{figure}

\begin{figure}[t]
	\centering
	\includegraphics[width=1.0\linewidth]{figures/feature_visualization_v2.pdf}
	\caption{
    % Feature map comparisons with CoModGAN~\cite{comodgan}. We visualize encoder features, globally modulated features and spatially modulated feature, at the resolution of $256\times256$.
    Visualization of the encoder feature map, globally modulated feature map and spatially modulated feature map, at the resolution $256\times256$.
	}
	\label{fig:feature}
	\vspace*{-.15in}
\end{figure}

Due to the limited expressive power of the global vector $\vg$ on representing $2$-d visual details, and the inconsistent features inside and outside the hole~\cite{deepfillv2,liu2018image}, the global modulation may generate distorted features inconsistent with the context, as visualized in \cref{fig:feature}.
To compensate for this limitation, we propose a spatial modulation stage at each decoder level. The visualization in \cref{fig:feature} shows that the feature maps after applying spatial modulation generates much more reasonable features.
Specifically, the spatial modulation takes $\tX$ as the spatial code and $\vg$ as the global code to modulate the input local feature $\tF_l^{(i)}$ in a spatially adaptive fashion.
However, different from existing spatial modulation methods~\cite{spade,stylemapgan,albahar2021pose}, our approach is based on a new \emph{spatial modulation-demodulation} mechanism to avoid the potential ``water droplet'' artifact~\cite{stylegan2} caused by instance normalization.
As shown in \cref{fig:modulation}, the spatial modulation follows a \emph{modulation-convolution-demodulation} pipeline:
\begin{itemize}
    % \setlength\itemsep{0em}
    % \itemsep-1em 
    \item \emph{Spatial modulation}. 
    A spatial tensor $\tA_0 = \APN(\tY)$ is produced from feature $\tX$ by a 2-layer convolutional affine parameter network (APN). 
    Meanwhile, a global vector $\valpha = \fc(\vg)$ is produced from global code $\vg$ with a fully connected layer ($\fc$) to capture global context. A final spatial tensor $\tA = \tA_0 + \valpha$ is then the boardcast summation of $\tA_0$ and $\valpha$ for scaling the intermediate feature $\tY$ of the spatial modulation block with element-wise product $\odot$:
        \begin{align}
        \label{eq:modulation_scale2}
            \bar{\tY} &= \tY \odot \tA.
        \end{align}
    \item \emph{Convolution}. The modulated tensor $\hat{\tX}$ is convolved with a $3\times3$ learnable kernel $\tK$, resulting in $\hat{\tY}$
        \begin{align}
        \label{eq:conv}
            \hat{\tY} &= \bar{\tY} \ast \tK.
        \end{align}
    \item \emph{Spatially-aware demodulation}. In this step, we generalize the demodulation step of StyleGAN2~\cite{stylegan2} to compute the normalized output $\widetilde{\tY}$. Specifically, we assume that the input features $\tY$ are independent random variables with unit variance and after the modulation, the expected variance of the output is not changed, \ie $\displaystyle  \E_{\ry \in \widetilde{\tY}} [\Var(\ry)]&=1$.
        % \begin{align}
        % % \label{eq:assumption}
        %     % \displaystyle  \E_{\rx \in \tX} [\Var(\rx)]&=1 \\
        %     \label{eq:assumption2}
        %     \displaystyle  \E_{\ry \in \widetilde{\tY}} [\Var(\ry)]&=1.
        % \end{align}
    This assumption gives the demodulation computation:
        \begin{align}
        \label{eq:demodulation}
        \widetilde{\tY} &= \hat{\tY} \odot \tD,
        \end{align}
    where $\tD = 1 / \sqrt{\tK^2 \odot \E_{\va \in \tA}[\va^2]}$ is demodulation coefficient. \cref{eq:demodulation} is implemented with standard tensor operations. Please refer to the more details in the supplementary material.
    % \todo{revise supp material.} 
    \item \emph{Adding spatial bias and broadcast noise}.
    The normalized feature $\widetilde{\tY}$ is added to a shifting tensor $\tB = \APN(\tX)$ produced by another affine parameter network (APN) from feature $\tX$ along with the broadcast noise $\vn$ to produce the new local feature $\tF_l^{(i+1)}$:
    \begin{align}
    \label{eq:modulation_shift}
        % \tB = \APN(\tX), \\
        \tF_l^{(i+1)} = \widetilde{\tY} + \tB + \vn.
    \end{align}
\end{itemize}

\noindent \textbf{Expanding the Receptive Field at Early Stage.} \quad
The fully convolutional models suffer from slow growth of effective receptive field~\cite{luo2016understanding}, especially at the early stage of the network.
For this reason, our encoder based on strided convolution usually generate invalid features inside the hole region, making the feature correction at decoding stage more challenging.
A recent work~\cite{lama} show that fast Fourier convolution (FFC)~\cite{chi2020fast} can help early layers to achieve receptive field that covers an entire image.
However, the work~\cite{lama} stacks FFC at the bottleneck layer which is computationally demanding. Moreover, like many other works~\cite{deepfillv2}, the shallow bottleneck layer cannot capture global semantic effectively.
We propose to replace the convolutional block with FFC for the encoder layers. FFC enables the encoder to propagate features at early stage and thus address the issue of generating invalid features inside the hole, which helps improve the results as shown in the ablation study in Tab.~\ref{tab:ablation}. 

%==> we have comparison without FFC
%\es{Is this actually helping the quality and results? If yes, should ablate. If not, or negligibly, I proposed to remove.}

% \noindent \textbf{The.} \quad
% \todo{finish that part}
% The positional encoding on an image of resolution $H\times W$ is defined as the concatenate of Fourier feature:
% \begin{align}
% \label{eq:pe}
% PE = \frac{1}{\sqrt{2}}[\sin(x), \cos(x)],
% \end{align}
% where the constant $\frac{1}{\sqrt{2}}$ is to ensure the variance of input is $1$ \todo{double-check}.
% To enhance structural awareness of our inpainting model, we concatenate the positional encoding to input of the generator, as well as the intermedia layer of the encoder. The positional encoding provide side information for model to reconstruct lines and repeating structures.


\begin{figure*}[t]
	\centering
	\includegraphics[width=1.\linewidth]{figures/mask.pdf}
	\caption{Examples of our object-aware masks generated for training (left) in comparison to the real inpainting request (right) and the mask generated by CoModGAN~\cite{comodgan}. Note that our masks are more consistent with real user requests.
	}
	\label{fig:mask}
	\vspace*{-.15in}
\end{figure*}


\subsection{Object-aware Training}
\label{sec:mask_scheme}
The algorithm to generate mask for training is crucial. In essence, the sampled masks should be similar to the masks drawn in realistic use-cases. Previous works generate square-shaped masks~\cite{pathak2016context,iizuka2017globally} or use random strokes~\cite{partial_convolutions} or a mixture of both~\cite{deepfillv2,comodgan} for training.
A recent work~\cite{profill} overlays object-shaped holes on salient objects of input images to mimic the object removal use-case.
However, since foreground objects are always occluded from the mask, such a scheme ignores the use-case of object completion, \ie reconstructing an object from a partially masked one. Furthermore, saliency detection only predicts the most obvious object while ignoring the surrounding objects, causing ambiguity to the training.

To better support realistic object removal use cases while preventing the model from generate new objects inside the holes, we propose an object-aware training scheme that generate more realistic masks during training as shown in \cref{fig:mask}. 
Specifically, we first pass the training images to PanopticFCN \cite{li2021fully} to generate highly accurate instance-level segmentation annotations. Next, we sample a mixture of free-form hole~\cite{comodgan} and object hole~\cite{profill} as the initial mask. Finally, we compute the overlapping ratio between the hole and each thing instance from an image. If the overlapping ratio is larger than a threshold, we exclude the foreground instance from the hole. Otherwise, the hole is unchanged to mimic object completion. We set the threshold to $0.5$. We dilate and translate the object mask randomly to avoid overfitting. We also dilate the hole on the instance segmentation boundary to avoid leaking background pixel near the hole into the inpainting region. Please refer to the supplementary material for more details.


% Realistic inpainting requests from users usually focus on background object removal and partial object completion as shown in Figure 1 left. However, the CoModGAN leverage randomly generated mask for model training, as shown in Figure 1 right. To bridge the generalization gap while allowing the model to focus on background object removal and partial object completion, we pre-compute the instance segmentation on training image via the PanopticFCN~\cite{panopticFCN} and design a new mask generation pipeline as follows:
% \begin{itemize}
%     \item We sample an initial mask m0, which can be either a CoModGAN mask or an object mask. To sample the CoModGAN mask, we follow the default procedure as elaborated by CoModGAN. To sample the object mask, we randomly chose an object mask from an object mask dataset and apply random translation and dilation to the mask.
%     \item We compute the overlapping ratio $r_i=overlap(m0,s_i)$ between each segment of foreground instance $s_i$ and the generated mask m0. If the overlapping ratio is larger than 0.5, we exclude $s_i$ from m0 so that the mask avoids the foreground object. 
% \end{itemize}
% Please refer to the appendix for the pseudo code of the implementation.


\subsection{The Training Objective}
\label{sec:training_goal}
Our generator is trained with a combination of adversarial loss~\cite{comodgan} and perceptual loss~\cite{lama}. The experiments show that our method can also achieve good results when purely using the adversarial loss as in~\cite{comodgan}, but adding the perceptual loss can further improve the performance significantly. 

% leverage a pretrained semantic segmentation model to compute the perceptual loss, encourage semantic-level reconstruction.

\subsection{The Masked-$R_1$ Regularization}
\label{sec:masked_r1}
To stabilize the adversarial training, we leverage $R_1$ regularization~\cite{mescheder2018training} to penalize the discriminator from overfitting during training.
However, different from the existing works~\cite{comodgan,lama} that naively apply the $R_1$ regularization, we propose a masked-$R_1$ regularization specifically designed for inpainting:
\begin{align}
\label{eq:masked_r1}
    \bar{R}_1 = \frac{\gamma}{2} \displaystyle  \E_{p_{\rm{data}}}[\norm{m \odot \nabla D(x)}^2],
\end{align}
where $m$ is the mask indicating the hole region and $\gamma$ is a balancing weight.
Different from the previous $R_1$ regularization~\cite{mescheder2018training}, \cref{eq:masked_r1} leverages the mask $m$ to avoid computing the gradient penalty inside the mask. This eliminates the potential harmful impact of computing regularization outside the holes, and therefore stabilizes the training.

